A Dynamic By-example BTF Synthesis Scheme

Measured Bidirectional Texture Function (BTF) can faithfully reproduce a realistic appearance but is costly to acquire and store due to its 6D nature (2D spatial and 4D angular). Therefore, it is practical and necessary for rendering to synthesize BTFs from a small example patch. While previous methods managed to produce plausible results, we find that they seldomly take into consideration the property of being dynamic, so a BTF must be synthesized before the rendering process, resulting in limited size, costly pre-generation and storage issues. In this paper, we propose a dynamic BTF synthesis scheme, where a BTF at any position only needs to be synthesized when being queried. Our insight is that, with the recent advances in neural dimension reduction methods, a BTF can be decomposed into disjoint low-dimensional components. We can perform dynamic synthesis only on the positional dimensions, and during rendering, recover the BTF by querying and combining these low-dimensional functions with the help of a lightweight Multilayer Perceptron (MLP). Consequently, we obtain a fully dynamic 6D BTF synthesis scheme that does not require any pre-generation, which enables efficient rendering of our infinitely large and non-repetitive BTFs on the fly. We demonstrate the effectiveness of our method through various types of BTFs taken from UBO2014.

==> 5_implemention.tex <==
\section{Implementation}



\paragraph{Importance Sampling}
Importance sampling is crucial to efficient rendering. However, we are not focusing on developing a new importance sampling strategy, as we consider it orthogonal to our main objective. Instead, we employ a straightforward cosine-weighted hemisphere sampling to our method. Previous work as predicting a histogram distribution~\cite{zhu:2021:complexLum,Xu:2023:neuSample} or using normalizing flows~\cite{Xu:2023:neuSample} can be adapted to our method. 
\paragraph{Parallax Effects}
Incorporating offset~\cite{kuznetsov:2021:neumip} into neural materials provides a method for achieving a pseudo-3D effect on 2D surfaces. 
To obtain a parallax effect, previous work either implicitly estimates a 4D offset from BTFs~\cite{kuznetsov:2021:neumip,fan:2023:BTF} or explicitly creates a 7D synthetic SBTF (Silhouette BTF) dataset for training~\cite{kuznetsov:2022:neumip2}. 
Considering the measured BTF datasets do not include the offset data, obtaining the additional parallax effect involves an unstable, unsupervised learning process~\cite{kuznetsov:2021:neumip}. Consequently, we chose to exclude parallax effects from our method, a decision that does not impact the validity of our conclusions.

The detailed implementation of training and rendering integration is described in the supplementary material.
% However, in our case, the measured BTF often does not exhibit a significant parallax effect. 
% Employing an additional estimated implicit offset module results in minor visual differences and causes unworthy performance loss.
% From another perspective, learning an SBTF involves creating a 7D synthetic dataset, which is not compatible with the measured BTFs.
% Moreover, we consider the parallax effects to be incremental to our method, without it does not affect the conclusion of our method. 
% Therefore, we decide not to include parallax effects in our method. 
% However, it does not mean our proposed dimension reduction method can not handle 4D offset function ($\mathbf{offset}(\uv, \wi)$). We conducted a minor experiment on a synthetic offset dataset in \todo{Sec.xxx}, which shows that our method is general for decomposing data.

% \input{tabs/tab_runtime}


==> figs/ablation.tex <==
\begin{figure}[t]
	\centering
	%\setlength{\resLen}{1.1in}
	\addtolength{\tabcolsep}{-3.5pt}
	\small
	\begin{tabular}{ccccc}
        \raisebox{0.35in}{\rotatebox[origin=c]{90}{\textsc{Wood06}}} &
    	\begin{overpic}[width=0.23\columnwidth]{pics/ablation/d8.png}
            \put(2, 2){\color{white}\small{0.06893}}
            \end{overpic} &
            \begin{overpic}[width=0.23\columnwidth]{pics/ablation/ours.png}
            \put(2, 2){\color{white}\small{0.06068}}
            \end{overpic} &
            \begin{overpic}[width=0.23\columnwidth]{pics/ablation/d32.png}
            \put(2, 2){\color{white}\small{0.07289}}
            \end{overpic} &
            \begin{overpic}[width=0.23\columnwidth]{pics/ablation/gt.png}
            \end{overpic}
	  \\
        & Ours (D8) & Ours (D16) & Ours (D32) & GT
        \\
        \raisebox{0.35in}{\rotatebox[origin=c]{90}{\textsc{Leather08}}} &
    	   \begin{overpic}[width=0.23\columnwidth]{pics/ablation/l3.png}
            \put(2, 2){\color{white}\small{0.06998}}
            \end{overpic} &
            \begin{overpic}[width=0.23\columnwidth]{pics/ablation/ours.png}
            \put(2, 2){\color{white}\small{0.06068}}
            \end{overpic} &
            \begin{overpic}[width=0.23\columnwidth]{pics/ablation/l5.png}
            \put(2, 2){\color{white}\small{0.06371}}
            \end{overpic} &
            \begin{overpic}[width=0.23\columnwidth]{pics/ablation/gt.png}
            \end{overpic}
	  \\
        & Ours (L3) & Ours (L4) & Ours (L5) & GT
	\end{tabular}
	\caption{\label{fig:ablation}
        Validation of our method's representation capability for different BTFs.  
        We visualize our results along with ground truth BTFs with two different pairs of directions for each different material. We use structural dissimilarity (DSSIM, lower is better) as the error metric (shown at the bottom-left). Our results are highly close to GT, demonstrating the capability of our method. 
	}
\end{figure}





==> figs/comp_btf_syn.tex <==
\begin{figure}[t]
	\addtolength{\tabcolsep}{-4.5pt}
	\small
	\begin{tabular}{cccc}
   	\raisebox{0.5in}{\rotatebox[origin=c]{90} {\textsc{Wood06}}} &
        \begin{overpic}[width=0.32\columnwidth]{pics/placeholder1x1.jpg}
             \put(65, 2){\includegraphics[width=0.1\columnwidth]{pics/placeholder1x1.jpg}}
                   \put(2, 2){\color{white}\small{ 0.059508}}
            \end{overpic} &
   	\begin{overpic}[width=0.32\columnwidth]{pics/placeholder1x1.jpg}
         \put(65, 2){\includegraphics[width=0.1\columnwidth]{pics/placeholder1x1.jpg}}
              \put(2, 2){\color{white}\small{0.043654}}
            \end{overpic} &
            \begin{overpic}[width=0.32\columnwidth]{pics/placeholder1x1.jpg}
            \put(79, 79){\includegraphics[width=0.06\columnwidth]{pics/placeholder1x1.jpg}}
            \end{overpic}  
	\\
    	\raisebox{0.5in}{\rotatebox[origin=c]{90} {\textsc{Leather08}}} &
 	\begin{overpic}[width=0.32\columnwidth]{pics/placeholder1x1.jpg}
                      \put(65, 2){\includegraphics[width=0.1\columnwidth]{pics/placeholder1x1.jpg}}
                   \put(2, 2){\color{white}\small{ 0.102273}}
            \end{overpic} &
   	\begin{overpic}[width=0.32\columnwidth]{pics/placeholder1x1.jpg}
            \put(65, 2){\includegraphics[width=0.1\columnwidth]{pics/placeholder1x1.jpg}}
            \put(2, 2){\color{white}\small{ 0.078400}}
            \end{overpic} &
            \begin{overpic}[width=0.32\columnwidth]{pics/placeholder1x1.jpg}
            \put(79, 79){\includegraphics[width=0.06\columnwidth]{pics/placeholder1x1.jpg}}
            \end{overpic}  
	\\
         & Ours w/ &  Ours w/  &  BTF Synthesis
        \\
        & Hist. preserving& Texture Quilting  & 
	\end{tabular}
	\caption{\label{fig:comp_btf_syn}
        Comparison with previous BTF synthesis methods. Note that none of the previous methods supports dynamic synthesis. They must do a pre-generation which limiteds.
	}
\end{figure}

==> figs/comp_gt_neumip.tex <==
\begin{figure*}[tb]
	\centering
	\addtolength{\tabcolsep}{-3.5pt}
	\small
	\begin{tabular}{cccc}
     	\raisebox{0.8in}{\rotatebox[origin=c]{90} {\textsc{Fabric12}}} &
    	\begin{overpic}[width=0.32\textwidth]{pics/comp_gt/ours.jpg}
            \end{overpic} &
            \begin{overpic}[width=0.32\textwidth]{pics/comp_gt/gt.jpg}
            \end{overpic} &
            \begin{overpic}[width=0.32\textwidth]{pics/comp_gt/ours.jpg}
            \end{overpic}
	\\
            &
            \begin{overpic}[width=0.24\columnwidth]{pics/comp_syn/crops/fabric12_neumip_repeat_A.jpg}\end{overpic} 
            \begin{overpic}[width=0.24\columnwidth]{pics/comp_syn/crops/fabric12_neumip_repeat_B.jpg}\end{overpic} &
            \begin{overpic}[width=0.24\columnwidth]{pics/comp_syn/crops/fabric12_ours_repeat_A.jpg}\end{overpic} 
            \begin{overpic}[width=0.24\columnwidth]{pics/comp_syn/crops/fabric12_ours_repeat_B.jpg}\end{overpic} &
            \begin{overpic}[width=0.24\columnwidth]{pics/comp_syn/crops/fabric12_neumip_histo_A.jpg}\end{overpic} 
            \begin{overpic}[width=0.24\columnwidth]{pics/comp_syn/crops/fabric12_neumip_histo_B.jpg}\end{overpic}
        \\
    	\raisebox{0.8in}{\rotatebox[origin=c]{90} {\textsc{Leather03}}} &
    	\begin{overpic}[width=0.32\textwidth]{pics/comp_syn/leather03_neumip_repeat.jpg}
            \end{overpic} &
            \begin{overpic}[width=0.32\textwidth]{pics/comp_syn/leather03_ours_repeat.jpg}
            \end{overpic} &
            \begin{overpic}[width=0.32\textwidth]{pics/comp_syn/leather03_neumip_histo.jpg}
            \end{overpic}
	\\
            &
            \begin{overpic}[width=0.24\columnwidth]{pics/comp_syn/crops/leather03_neumip_repeat_A.jpg}\end{overpic} 
            \begin{overpic}[width=0.24\columnwidth]{pics/comp_syn/crops/leather03_neumip_repeat_B.jpg}\end{overpic} &
            \begin{overpic}[width=0.24\columnwidth]{pics/comp_syn/crops/leather03_ours_repeat_A.jpg}\end{overpic} 
            \begin{overpic}[width=0.24\columnwidth]{pics/comp_syn/crops/leather03_ours_repeat_B.jpg}\end{overpic} &
            \begin{overpic}[width=0.24\columnwidth]{pics/comp_syn/crops/leather03_neumip_histo_A.jpg}\end{overpic} 
            \begin{overpic}[width=0.24\columnwidth]{pics/comp_syn/crops/leather03_neumip_histo_B.jpg}\end{overpic}
	\\
            & Ours  & Ours & Ours \\
        & (NeuMIP w/ repetitive tiling) & (NeuMIP w/ hist. preserving) & (Improved Biplane w/ hist. preserving)
	\end{tabular}
	\caption{
            \label{fig:comp_syn}
            We implement NeuMIP with histogram preserving blending (third column) to demonstrate our BTF synthesis scheme is general to any BTF dimension reduction method with an accessible positional feature plane.
            % Comparison between NeuMIP~\cite{kuznetsov:2021:neumip} and ours.
            % Since our synthesis scheme is general to neural BTF representation methods with an accessible positional feature plane, we can easily extend the synthesis scheme to NeuMIP (the third column). 
            Our method (second and fourth columns) shows great effectiveness in both representation and synthesis. NeuMIP, however, notably lacks high-frequency details, resulting in unsharp highlights (\textsc{Stone04}) and blurred reflections (\textsc{Leather03}). 
            % 
            % \added{Beibei: why our representation model is better than NeuMIP? this need a deep analysis.  }
            % \todo{Analysis on the result}
            % We conduct the comparison on various materials, including carpet, leather, fabric, etc. These materials are from the UBO2014~\cite{weinmann:2014:ubo14} measured BTF dataset.
            % Specifically, in the Ball Scene w/ Leather08, Neumip fails to capture the highlight details near the scratches on the leather, whereas our method preserves them very well.
             % \junqiu{jacket scene good good!}
             % Although NeuMIP only supports repetitive tiling, which produces unrealistic repetition, our synthesis scheme can be extended to NeuMIP (the third column) to make a fair comparison. 
            % Our method shows great effectiveness in both representation and synthesis. \added{Beibei: why our representation model is better than NeuMIP? this need a deep analysis
        }
\end{figure*}


==> figs/sup_res.tex <==
\begin{teaserfigure}
	\addtolength{\tabcolsep}{-5.0pt}
    \begin{tabular}{ccccc}
        \begin{overpic}[width=0.24\textwidth]{pics/sup/carpet01_1.jpg}
        \put(2, 2){\color{white}\large{\textsc{Carpet01}}}
        \end{overpic} &
        \begin{overpic}[width=0.24\textwidth]{pics/sup/carpet01_2.jpg}
         \put(78, 78){\includegraphics[width=0.05\columnwidth]{pics/teaser/carpet01.jpg}}
        \end{overpic} & \, &
        \begin{overpic}[width=0.24\textwidth]{pics/sup/carpet02_1.jpg}
        \put(2, 2){\color{white}\large{\textsc{Carpet02}}}
        \end{overpic} &
        \begin{overpic}[width=0.24\textwidth]{pics/sup/carpet02_2.jpg}
         \put(78, 78){\includegraphics[width=0.05\columnwidth]{pics/teaser/carpet02.jpg}}
        \end{overpic} \\
        \begin{overpic}[width=0.24\textwidth]{pics/sup/carpet03_1.jpg}
        \put(2, 2){\color{white}\large{\textsc{Carpet03}}}
        \end{overpic} &
        \begin{overpic}[width=0.24\textwidth]{pics/sup/carpet03_2.jpg}
         \put(78, 78){\includegraphics[width=0.05\columnwidth]{pics/teaser/carpet03.jpg}}
        \end{overpic} & \, &
        \begin{overpic}[width=0.24\textwidth]{pics/sup/carpet04_1.jpg}
        \put(2, 2){\color{white}\large{\textsc{Carpet04}}}
        \end{overpic} &
        \begin{overpic}[width=0.24\textwidth]{pics/sup/carpet04_2.jpg}
         \put(78, 78){\includegraphics[width=0.05\columnwidth]{pics/teaser/carpet04.jpg}}
        \end{overpic} \\
        \begin{overpic}[width=0.24\textwidth]{pics/sup/felt05_1.jpg}
        \put(2, 2){\color{white}\large{\textsc{Felt05}}}
        \end{overpic} &
        \begin{overpic}[width=0.24\textwidth]{pics/sup/felt05_2.jpg}
         \put(78, 78){\includegraphics[width=0.05\columnwidth]{pics/teaser/felt05.jpg}}
        \end{overpic} & \, &
        \begin{overpic}[width=0.24\textwidth]{pics/sup/felt09_1.jpg}
        \put(2, 2){\color{white}\large{\textsc{Felt09}}}
        \end{overpic} &
        \begin{overpic}[width=0.24\textwidth]{pics/sup/felt09_2.jpg}
         \put(78, 78){\includegraphics[width=0.05\columnwidth]{pics/teaser/felt09.jpg}}
        \end{overpic}\\
        \begin{overpic}[width=0.24\textwidth]{pics/sup/leather01_1.jpg}
        \put(2, 2){\color{white}\large{\textsc{Leather01}}}
        \end{overpic} &
        \begin{overpic}[width=0.24\textwidth]{pics/sup/leather01_2.jpg}
         \put(78, 78){\includegraphics[width=0.05\columnwidth]{pics/teaser/leather01.jpg}}
        \end{overpic} & \, &
        \begin{overpic}[width=0.24\textwidth]{pics/sup/stone04_1.jpg}
        \put(2, 2){\color{white}\large{\textsc{Stone04}}}
        \end{overpic} &
        \begin{overpic}[width=0.24\textwidth]{pics/sup/stone04_2.jpg}
         \put(78, 78){\includegraphics[width=0.05\columnwidth]{pics/teaser/stone04.jpg}}
        \end{overpic}
        % \begin{overpic}[width=0.24\textwidth]{pics/sup/wallpaper11_1.jpg}
        % \put(2, 2){\color{white}\large{\textsc{Wallpaper11}}}
        % \end{overpic} &
        % \begin{overpic}[width=0.24\textwidth]{pics/sup/wallpaper11_2.jpg}
        % \end{overpic} & \, &
        % \begin{overpic}[width=0.24\textwidth]{pics/sup/stone10_1.jpg}
        % \put(2, 2){\color{white}\large{\textsc{Stone10}}}
        % \end{overpic} &
        % \begin{overpic}[width=0.24\textwidth]{pics/sup/stone10_2.jpg}
        % \end{overpic} \\
	\end{tabular}
  \vspace{-8mm}
  \caption{We propose a novel by-example BTF synthesis scheme that can dynamically synthesize a non-repetitive, infinite large BTF from a small example BTF ($400 \times 400$). 
  To further demonstrate our method's effectiveness in both synthesis and rendering, we provide our results with histogram-preserving blending~\cite{heitz:2018:histo} on eight BTFs from UBO2014~\cite{weinmann:2014:ubo14} BTF dataset. Each BTF is rendered under two different lighting conditions. Our method can synthesize an infinitely large, non-repetitive BTF while faithfully reproducing the appearance across various types of materials.
  }
  \Description{BTF Synthesis.}
  \end{teaserfigure}


==> figs/valid_mip.tex <==
\begin{figure}[t]
	\centering
	%\setlength{\resLen}{1.1in}
	\addtolength{\tabcolsep}{-3.5pt}
	\small
	\begin{tabular}{cccc}
    	\raisebox{0.45in}{\rotatebox[origin=c]{90}{\textbf{Ours}}} &
    	\begin{overpic}[width=0.28\columnwidth]{pics/valid_mip/leather11_71_4_ 0.04860_pred.jpg}
            \put(2, 2){\color{white}\small{ 0.04860}}
            \end{overpic} &
            \begin{overpic}[width=0.28\columnwidth]{pics/valid_mip/leather11_71_8_ 0.04163_pred.jpg}
            \put(2, 2){\color{white}\small{ 0.04163}}
            \end{overpic} &
            \begin{overpic}[width=0.28\columnwidth]{pics/valid_mip/leather11_71_16_ 0.05722_pred.jpg}
            \put(2, 2){\color{white}\small{ 0.05722}}
            \end{overpic} 
            % &
            % \begin{overpic}[width=0.22\columnwidth]{pics/valid_mip/wallpaper12_52_16_0.022782441641685913_pred.jpg}
            % \put(2, 2){\color{white}\small{ 0.02278}}
            % \end{overpic}
	\\
     	\raisebox{0.45in}{\rotatebox[origin=c]{90}{\textbf{GT}}} &
    	\begin{overpic}[width=0.28\columnwidth]{pics/valid_mip/leather11_71_4_ 0.04860_gt.jpg}
            \put(2, 2){\color{white}{\textsc{Leather11}}}
            \end{overpic} &
            \begin{overpic}[width=0.28\columnwidth]{pics/valid_mip/leather11_71_8_ 0.04163_gt.jpg}
            % \put(2, 2){\color{black}\small{ 0.43911}}
            \end{overpic} &
            \begin{overpic}[width=0.28\columnwidth]{pics/valid_mip/leather11_71_16_ 0.05722_gt.jpg}
            % \put(2, 2){\color{black}\small{ 0.42372}}
            \end{overpic} 
            % &
            % \begin{overpic}[width=0.22\columnwidth]{pics/valid_mip/wallpaper12_52_16_0.022782441641685913_gt.jpg}
            % % \put(8, 4){\color{white}\small{\emph{Wallpaper12}}}
            % \end{overpic}
	\\
         & LoD 2 ($100 \times 100$) & LoD 3 ($50 \times 50$) & LoD 4 ($25 \times 25$)
         % & LoD 4
	\end{tabular}
	\caption{\label{fig:valid_mipmap}
        Validation of our method's capability to create precise mipmap in the positional feature plane. The mipmapping is done on the 2D positional feature plane instead of the recovered 6D BTF result and the resolution of the finest level is $400 \times 400$. Each image is resized by the nearest interpolation. The DSSIM is shown at the bottom-left. Our method faithfully preserved the appearance even at high levels. 
	}
\end{figure}




